A Bayesian approach to the modelling of alpha Cen A

Determining the physical characteristics of a star is an inverse problem consisting in estimating the parameters of models for the stellar structure and evolution, knowing certain observable quantities. We use a Bayesian approach to solve this problem for alpha Cen A, which allows us to incorporate prior information on the parameters to be estimated, in order to better constrain the problem. Our strategy is based on the use of a Markov Chain Monte Carlo (MCMC) algorithm to estimate the posterior probability densities of the stellar parameters: mass, age, initial chemical composition,... We use the stellar evolutionary code ASTEC to model the star. To constrain this model both seismic and non-seismic observations were considered. Several different strategies were tested to fit these values, either using two or five free parameters in ASTEC. We are thus able to show evidence that MCMC methods become efficient with respect to more classical grid-based strategies when the number of parameters increases. The results of our MCMC algorithm allow us to derive estimates for the stellar parameters and robust uncertainties thanks to the statistical analysis of the posterior probability densities. We are also able to compute odds for the presence of a convective core in alpha Cen A. When using core-sensitive seismic observational constraints, these can raise above ~40%. The comparison of results to previous studies also indicates that these seismic constraints are of critical importance for our knowledge of the structure of this star.

==> Sections/Bayes.tex <==
\section{The Bayesian methodology}





==> Sections/Discussion.tex <==
\subsection{Comparison with previous studies}


In this section we briefly compare our results to previous studies using seismic data for {\acena} \citep{Eggenberger04,Miglio05}. It is important to first stress the methodological differences between these previous works and ours. They both rely on optimization approaches, and none of them in a Bayesian framework. This poses obvious problems when comparing the results. First, it is not clear how fixing the mass compares with our use of a Gaussian prior. More importantly, without access to the PPDs of the parameters, it is not possible to assess whether or not the maximum values reported in these works correspond to local or global extrema. We already saw in Sect.~\ref{sect:simu5D} that some PPDs were difficult to sample (in the 5-dimensional case, with $\Xv = (L,\teff,R,\als)$ and a Gaussian prior on the mass), therefore such a configuration might not be uncommon.

Different physics were also used in the stellar codes. The major point is that both studies used microscopic diffusion, which we have neglected. This should have an observable effect, but its nature remains difficult to anticipate. Gravitational settling will deplete the external convective zone of its heaviest elements. The intial metallicity might thus be increased, or the initial hydrogen mass fraction decreased, in order to reproduce the observed $Z/X$. The impact of this additional mechanism shall be studied with care in future studies using the MCMC approach.

Finally, {\acenb} has been modelled simultaneously in these studies. This introduces additional constraints on the solution to the inverse problem. We did not retain this strategy for logistical reasons. Modelling two stars at the same time would have implied significant modifications in our code. We thus prefered to focus on the star with the most reliable data (in particular the seismic data).

We should also consider the effect of the value they used for the average large separation, $\ass = 8.7 \pm 0.8$~$\mu$Hz used in these studies. To evaluate rapidly the impact this has on the estimate of the age, we can use the grid described in Sect.~\ref{sect:grids5D}. We obtain a relatively Gaussian marginal PPD and a lower age $\stage = 3.84 \pm 0.61$~$\mu$Hz for $\Xv = (L,\teff,R,\ass)$ and the Gaussian prior on the mass. Note that if we use the value provided by \citet{deMeulenaer10}, $\ass = 5.8 \pm 0.1$~$\mu$Hz we obtained $\stage = 6.04 \pm 0.35$~$\mu$Hz for the same $\Xv$ and prior. This agrees with the theoretical behaviour of the small separation, decreasing with age. We should however recall that if these grid-based are convenient because easily computed once the grid has been produced, we are still affected by the drawbacks we mentioned in Sect.~\ref{sect:grids5D}. The marginal PPDs for the $Z_0$, $\alpha$ and $X_0$ are obviously problematic and a proper MCMC simulation would be necessary (or a denser grid on larger scales) would be necessary to provide acceptable estimates of these parameters. 

Keeping in mark these remarks, we see that for the age of {\acena} we estimate in the 5-dimensional (runs \#12 and \#13) is significantly lower than those quoted in \citet{Miglio05}. Their A1e model seems to be the more relevant for a comparison with our own results. They obtain an age of $6.7\pm0.5$~Gyr. This is the main departure between the two studies. The other parameters are all within their respective error bars (which are, as a general rule comensurate). However, given the complex interplay between the stellar parameters and other variables such as, for instance, $\xc$, a change in one of them, even within the quoted error bars might very well lead to a much significant departure of another parameter. Only an homogeneous comparison using both models, with the same physical prescriptions can give us more information on the differences between our studies. The same kind of picture can be drawn from a comparison between our work and the results of \citet{Eggenberger04}


The problem of the uncertainties is also difficult to tackle. As a general rule, those from \citet{Eggenberger04} seem to be underestimated with respect to ours. However their method for estimating credible intervals is much less robust and statistically sound than what is allowed from the study of the marginal PPDs of the stellar parameters. \citet{Miglio05} used a Hessian-based approach and obtained uncertainties commensurate with ours. Our study also provide a confirmation to theirs since they need to make the implicit assumption that they are dealing with Gaussian PPD before inverting their Hessian matrix. Note also that if this is not the case, this methodology is known to underestimate the uncertainties.

One could also contend that the differences come from the physics in our models, in particular the use of the EFF equation of state. This is unlikely since we see in \citet{Miglio05} that a change of equation of state only modestly affects the final estimates. Therefore, we suggest that most of the difference should be attributed to the adopted value for $\ass$.

Finally, we note that gyrochronology allows to obtain some measurements of the age of the stars. One should note that these could have been used as a prior on the age. We chose not to do so, in particular because we preferred to constrain the age using seismic quantities rather than by the use of gyrochronology. Nevertheless, we note that our estimates using the average small separations give an age in agreement with the results from \citet{Barnes07}. On the other hand, the estimates from \citet{Delorme11} are much higher and agree more closely with our estimates using $\als$. It is an interesting fact that the same technique provide with such different estimates.





==> Sections/Subsections/Specific.tex <==
\subsection{Specificity of the stellar parametric estimation}{\label{sect:specif}}

\subsubsection{Non-linearity}
\label{subsubsec:nonlinear}

\indent \indent Several methodologies have been used to estimate stellar parameters, ranging from grid-based optimisation \citep[e.g.][]{Morel00,Eggenberger04} to Bayesian analysis \citep[e.g.][]{Pont04,Jorgensen05}. Classical methods for optimisation are difficult to apply to highly non-linear models, in particular because the solution to the problem can be degenerate \citep[e.g.][]{Bazot04,Jorgensen05}. 

For a given metallicity and mixing-length parameter, the most important feature of the stellar structure in regard to non-linearity is certainly the presence or not of a convective core. Stars with central regions in full radiative equilibrium tend to evolve towards higher temperatures (right side of the HR-diagram, see Fig.~\ref{fig:erglim}) and luminosities. Evolutionary tracks corresponding to different masses do not cross during the earlier evolution stages, the Main-Sequence and the Subgiant Branch. On the contrary, stars with a convective core will exhibit evolutionary tracks bending towards lower temperatures and frequently crossing with those of other, less-massive, stars. This kind of behaviour can lead to multiple sets of parameters reproducing the exact same point in the HR-diagram, hence to the existence of multiple solutions to the optimisation problem.



\subsubsection{The Giant Branch}\label{sect:gb}

\indent \indent Using an MCMC algorithm to estimate stellar parameters of main-sequence or subgiant stars also poses the problem of the location of the Giant Branch (GB).\commSB{This sentence is not clear for me.} During this stage of evolution, low-mass stars (i.e. $\lesssim$2.3~\msol), are burning hydrogen in a shell surrounding a degenerate isothermal helium core. The evolutionary tracks roughly follow the Hayashi line and the luminosity increases fast with the stellar age \citep{Hayashi61}.

Obviously, we are not interested in computing too many models on the GB. They are indeed located far away from the locus of interest in the HR-diagram as defined by the observations. In fact they usually lie so far away from it that the probability for the MCMC algorithm to accept a model already on the GB is negligible. In other words, neglecting GB models should not affect the sampling of the PPD. This effect is increased by the fact that the surface metallicity of the star can also change if its convective envelop reaches the hydrogen burning shell, this would further increase the distance $\parallel \pmb{\mathscr{S}}(\thetav)-\Xv \parallel$ between theoretical values and observations in the data space ($\parallel . \parallel$ being a norm defined in this space).

The problem of computing models on the GB would not be so critical if the timescales for the different evolutionary stages were comparable. However, the main-sequence evolution is controlled by the hydrogen-burning timescale, $\tau_{MS} \approx 1$~Gyr. On the contrary, the lifetime of a star on the GB is much lower than that, of the order of a few million years. Consequently, the evolution code has to adopt much smaller timesteps when the star jumps to the GB, and the corresponding models are a lot more time-consuming to compute than main-sequence ones. Since we run typical Markov Chains with lengths $T=50000$, we cannot afford to waste too much time for models outside the Main-Sequence, or at least beyond the Subgiant region. 


To address this problem we used an adaptive boundary condition for the age parameter. The main difficulty if one wants to avoid the GB is to find its precise location in the HR diagram. For a given metallicity and mixing-length parameter, we know that the age at which the star will enter the giant phase decreases monotonically with increasing mass. We used this property to modify the domain of $\stage$ scanned by the MCMC algorithm. The maximum number of timesteps allowed for a given evolutionary sequence was fixed beforehand, so that it is large enough that it would certainly suffice to compute all possible models on the Main-Sequence and the Subgiant Branch. However, some models on the GB will require more timesteps than this maximum value, implying that the age of the last model computed in the sequence will be different than the age required by the trial parameter $\thetav^{\ast}$. In this case we select a new set of trial parameters without incrementing the Markov Chain and assign the incorrect trial set to $\thetav_{\mathrm{rej}}(=\{ t_{\mathrm{rej}}, M_{\mathrm{rej}} \} )$. We then change the limit of the space of parameters to be scanned, forbidding the algorithm to select trial parameters with ages higher than $t_{\mathrm{rej}}$ at masses lower than $M_{\mathrm{rej}}$. A series of $\thetav_{\mathrm{rej}}$ will therefore define an upper boundary for $\stage$ depending on the mass (see the dashed lines in both panels of Fig.~\ref{fig:erglim}). We note $\mathscr{D}_M(\stage)$ the domain of interest for the age parameter. In Fig.~\ref{fig:erglim} this domain appears in both panels as the non-shaded areas. The mapping from the space of parameters to the space of observable is such that only a small fraction of the former one is concern by the adaptive scheme. However, the right panel shows that we were able to reject a significant number of unuseful models. This method does not allow to reject all the GB models, however it helps to reduce the time spent in this region of the HR-diagram by the algorithm and ensures that we do not cut to sharply the domain of interest in age so that we could risk missing subgiant models that would be accepted by the MCMC algorithm, and which would thus be relevant in regard to the PPD estimation.

It is also noteworthy that this method does not modify the control properties of the chain, since the rejected models are never taken into account. Furthermore, it might only work when the upper boundary in the space of parameter is concave.


==> Tables/simu2D.tex <==
\begin{table*}[th!]
\begin{center}
\caption{Inferred stellar parameters constrained using non-seismic observables. First column: the number of the run, second column: observational constraints included in $\Xv$, third column: parameters for which a Gaussian prior has been used, fourth column: average mass (MAP value in brackets), fifth column: uncertainty on the mass, sixth column: average age (MAP value in brackets), seventh column: uncertainty on the age.}
\label{table:simu2D}
\begin{tabular}{lcccccc}
\hline %\hline

Run \#&$\Xv$&$\pi(M)$& $\hat{M}$ ({\msol})&$\hat{\sigma}_M$ ({\msol})& $\hat{\stage}$ (Gyr) & $\hat{\sigma}_{\stage}$ (Gyr)\\

\hline

1&$[L, \teff]$&Uniform& 1.121 & 0.019 & 5.63 & 1.14 \\
&&&(1.119)&&(5.80)&\\

2 &$[L, \teff, R]$ &Uniform& 1.116 & 0.011 & 5.98 & 0.52 \\
&&&(1.116)&&(5.98)&\\

3&$[L, \teff]$&Gaussian& 1.107 & 0.007 & 6.47 & 0.44 \\
&&&(1.106)&&(6.53)&\\

4&$[L, \teff, R]$&Gaussian& 1.108 & 0.006 & 6.34 & 0.28 \\
&&&(1.108)&&(6.35)&\\

5&$[L, \teff, \delta \nu_{02}]$&Uniform& 1.129  & 0.011 & 5.15& 0.63 \\
&&&(1.129)&&(5.12)&\\

6&$[L,\teff,\langle \delta \nu\rangle]$&Uniform& 1.130 & 0.008 & 5.03 & 0.39 \\
&&&(1.131)&&(5.01)&\\

7&$[L, \teff, \Delta \nu_{n,l}]$&Uniform& 1.110 & 0.010 & 6.31 & 0.39 \\
&&&(1.110)&&(6.32)&\\

10&$[L, \teff, R, \delta \nu_{02}]$&Uniform& 1.123 & 0.010 & 5.69 & 0.45  \\
&&&(1.123)&&(5.67)&\\

11&$[L,\teff, R, \langle \delta \nu\rangle]$&Uniform& 1.130& 0.008 & 5.36 & 0.34 \\
&&&(1.129)&&(5.38)&\\

12&$[L,\teff,R,\delta \nu_{02},\Delta \nu_{n,l}]$&Uniform& 1.110 & 0.008 & 6.29 & 0.36 \\
&&&(1.109)&&(6.3)&\\

13&$[L,\teff,R,\delta \nu_{02}]$&Gaussian& 1.110 & 0.006 & 6.22 & 0.27 \\
&&&(1.111)&&(6.21)&\\

14&$[L, \teff, R, \langle \delta \nu \rangle]$&Gaussian& 1.116 & 0.006 & 5.98 & 0.25 \\
&&&(1.115)&&(6.00)&\\

15&$[L,\teff,R,\delta \nu_{02},\Delta \nu_{n,l}]$&Gaussian& 1.107 & 0.005 & 6.41 & 0.23 \\
&&&(1.107)&&(6.4)&\\

\hline
%\end{tabular*}
\end{tabular}
\end{center}
\end{table*}


==> Tables/simu2D_grid.tex <==
\begin{table*}
\begin{center}
\caption{Inferred stellar parameters using direct integration of the PPD from the grid of models described in Sect.~\ref{}}
\label{table:simu2D_grid}
\begin{tabular}{cccccc}
\hline %\hline


$\Xv$&$\pi(M)$& $M$ ({\msol})&$\sigma_M$ ({\msol})& $\stage$ (Gyr) & $\sigma_{\stage}$ (Gyr)\\

\hline

$[L, \teff]$                                &Uniform      &1.120 &0.020&5.67 &1.20\\
$[L, \teff, R]$                             &Uniform      &1.116 &0.012&5.99 &0.53\\
$[L, \teff]$                                &Gaussian     &1.107 &0.007&6.48 &0.44\\
$[L, \teff, R]$                             &Gaussian     &1.108 &0.006&6.34 &0.28\\
$[L, \teff, \delta \nu_{02}]$                &Uniform     &1.128 &0.011&5.16 &0.66\\
$[L,\teff,\langle \delta \nu\rangle]$        &Uniform     &1.131 &0.008&5.00 &0.39\\
$[L, \teff, \Delta \nu_{n,l}]$               &Uniform     &1.110 &0.010&6.32 &0.41\\
$[L, \teff, R, \delta \nu_{02}]$             &Uniform     &1.122 &0.010&5.69 &0.45\\
$[L,\teff, R, \langle \delta \nu\rangle]$    &Uniform     &1.130 &0.008&5.35 &0.35\\
$[L,\teff,R,\delta \nu_{02},\Delta \nu_{n,l}]$&Uniform    &1.110 &0.008&6.29 &0.36\\
$[L,\teff,R,\delta \nu_{02}]$                 &Gaussia    &1.110 &0.006&6.22 &0.27\\
$[L, \teff, R, \langle \delta \nu \rangle]$  &Gaussian    &1.115 &0.006&5.99 &0.25\\
$[L,\teff,R,\delta \nu_{02},\Delta \nu_{n,l}]$&Gaussia    &1.107 &0.005&6.41 &0.24\\

\hline
%\end{tabular*}
\end{tabular}
\end{center}
\end{table*}

